Collaboratively Patching Linked Data

Today's Web of Data is noisy. Linked Data often needs extensive preprocessing to enable efficient use of heterogeneous resources. While consistent and valid data provides the key to efficient data processing and aggregation we are facing two main challenges: (1st) Identification of erroneous facts and tracking their origins in dynamically connected datasets is a difficult task, and (2nd) efforts in the curation of deficient facts in Linked Data are exchanged rather rarely. Since erroneous data often is duplicated and (re-)distributed by mashup applications it is not only the responsibility of a few original publishers to keep their data tidy, but progresses to be a mission for all distributers and consumers of Linked Data too. We present a new approach to expose and to reuse patches on erroneous data to enhance and to add quality information to the Web of Data. The feasibility of our approach is demonstrated by example of a collaborative game that patches statements in DBpedia data and provides notifications for relevant changes.

==> chapters/.svn/tmp/50_related.tex <==
\section{Related Work}
\label{sec:related}

% Datenstruktur-Validatoren
In order to raise quality in linked data applications various work has concentrated on syntactical and logical consistency by providing validators for RDF and OWL, e.g., W3C's RDF validator\footnote{\url{http://www.w3.org/RDF/Validator/}}, vapour\footnote{\url{http://validator.linkeddata.org/vapour}}, and OWL Validator\footnote{\url{http://owl.cs.manchester.ac.uk/validator/}}. Data quality in linked data has been criticised, as e.g., Hogan et al.  analyzed typical errors and set up the RDF-Alert Service\footnote{\url{http://swse.deri.org/RDFAlerts/}} that checks for syntax and datatype errors to support publishers of linked data\cite{Hogan2010}. Nevertheless, recent analyses  provided by LODStats\footnote{\url{http://stats.lod2.eu/rdfdoc/?errors=1}} show that there still is a vast amount of erroneous linked datasets available\cite{Demter2012}. However validators are restricted to syntactical consistency and thus are not able to fulfill the following requirements: 
\begin{enumerate}
\item Recognize the false usage of properties and classes if their domain and/or range is too generic. Therefore, the RDF-Triple \small{(dbp:Apple \textit{dbo:hasKeyPerson} dbo:Chairman)} might be syntactically correct, if Chairman is of domain Person. From a user's point of view this might be incorrect because a person is expected.
\item Recognize false facts in datatype properties, as e.g., the birthdate of a person can be syntactically correct (xsd:date) but factual wrong.
\end{enumerate}

Since validators are useful to verify syntactical consistency and correctness, they can not detect semantic or factual mistakes that may appear obvious to a human. Therefore, an effective integration of human intelligence, i.e. crowdsourcing, is required. We address this issue by enabling interoperable exchange of user feedback on linked data resources. Until now this concept is sparsely present in linked data community


% Initiativen die inhaltliche Fehler beheben
% Initiativen die neue Informationen zu Daten hinzufügen, aber keine Referenz bieten dass sie Mehrwert zu einem Datenset erzeugt haben.

% Spiele: WhoKnows, Risq!, OntoGame
A number of games with a purpose (GWAP)\cite{Ahn2004} are available that harness human intelligence for various tasks by providing appropriate incencitives, as e.g., fun, competition, reputation, etc. \cite{Siorpaes2010}. Most GWAP's are social web applications designed for the generation of metadata e.g. for multimedia resources but do not publish linked data. %On the other hand big data providers for linked data, as e.g. the Europeana might collect user feedback but handle curation results only internally \cite{Haslhofer2011} 
Harnessing human intelligence for creating semantic content has been studied by Siopaes and  Simperl, who provide a collection of games\footnote{http://ontogame.sti2.at/games/} to build ontologies, annotating videoclips, or matching ontologies \cite{siorpaes2008,Siorpaes2010}. However these games generally concentrate on content enrichment rather than content curation. 
%We have already published on \textit{gamification} approaches that aim to clean up linked data before.

\whoknows{} is a simple Query and Answer game in the style of `Who Wants to Be a Millionaire?' published previously by our research group, and designed to detect flaws in DBpedia resources\cite{Waitelonis2011c}. Likewise, \risq{}\footnote{http://apps.facebook.com/hpi-risq/} is a game in the style of ''Jeopardy!'' that focuses on the evaluation and ranking of linked data properties about famous people. Both games are yet well accepted but lack of a standardized method to publish the obtained curation efforts. 

%%%% QUELLEN! +  URLS ergänzen!
We propose a linked data approach to describe changes made to linked data resources, in order to make these updates (additions or deletions) reusable by the community. Therefore efforts are related that consider provenance information and the description of update statements on linked data resources. In regard of provenance, the \textit{Provenance Vocabulary}\cite{Hartig2009} (prv)\footnote{\url{http://trdf.sourceforge.net/provenance/ns.html}} is designed to make the origin, creation and alteration of data transparent, but lacks for concepts that describe the update of certain RDF-Triples. In Respect of describing updates on graphs serveral ontologies have been defined, e.g. \textit{changeset} (cs)\footnote{\url{http://vocab.org/changeset/schema.html}}, the \textit{graph update ontology} (guo)\footnote{\url{http://webr3.org/specs/guo/}}, \textit{delta}\footnote{\url{http://www.w3.org/DesignIssues/Diff}}, and \textit{triplify}-update\footnote{\url{http://triplify.org/vocabulary/update}}. All of these are limited to express changes within semantic data or to express provenance of changes. Both approaches are not designed to promote and discuss and exchange curation efforts, since facilities to express relevance and types of updates do not exist. To our best knowledge none of these ontologies have been combined or extended to exchange curation information about linked data resources. 

% We belive a standardized method (ontology) for the exchange of curation efforts will be fuitful for a number of applications. 
In this paper a new approach is proposed to curate linked data collaboratively, as e.g., flaws in DBpedia-resources are hard to detect by automatic procedures. In fact one could argue that curation efforts should be applied directly to the original source, i.e. the online encyclopedia wikipedia\footnote{\url{http://www.wikipedia.org}}. The herein proposed approach differs because: 
It is not limited to DBpedia resources and can be also applied where no immediate transformation of data is possible, as e.g., demonstrated by the live-DBpedia\footnote{\url{http://live.dbpedia.org/}} approach\cite{Stadler2010}. Furthermore the method proposed in this paper supports the common practice to replicate original data dumps at local repositories, and therefore enables a more convenient handling of data in regards of performance, stability and integration issues.
% else?...


 % carry information on user feedback and e.g. corrections. But all of them have certain limitations 
%Ontologies to publish feedback

%In the area of the unique key approach, which is used to identify same patches some work was already done by  
%With respect to URI naming on the Web, Bouquet et al. [2006] argue for a centralised naming architecture for minting URI signifiers for the Web; we see such a centralised ??naming authority? as going against the ad-hoc, decentralised, scale-free nature of the Web.
%\textit{Bouquet, P., Stoermer, H., Mancioppi, M., and Giacomuzzi, D. (2006). OkkaM: Towards a Solution to the ?Identity Crisis? on the Semantic Web. In Proceedings of SWAP 2006, the 3rd Italian Semantic Web Workshop, volume 201 of CEUR Workshop Proceedings.}

%The Sindice and Sig.ma search systems internally use inverse-functional properties to find equivalent identifiers [Tummarello et al., 2007, 2009]. Sindice investigates some bespoke ?schema-level? reasoning to identify a wider range of inverse-functional properties [Tummarello et al., 2007]; 
%\textit{Tummarello, G., Cyganiak, R., Catasta, M., Danielczyk, S., and Decker, S. (2009). Sig.ma: Live views on the Web of Data. In Semantic Web Challenge (ISWC2009).
%Tummarello, G., Delbru, R., and Oren, E. (2007). Sindice.com: Weaving the Open Linked Data. In ISWC/ASWC, pages 552?565.} however, compared to our approach, they (i) do not use functional properties or cardinality constraints; (ii) would still miss equivalences where identifiers use the same value with different inverse-functional properties, and where, e.g., those properties are in an equivalence or subsumption relationship.



% Verschiedene Gruppen haben bereits nach Fehlertypen und deren Bereinigung gesucht, z.B.
	% Pedantic Web Group: Untersuchte die Fehler und klassifizierte , es sind auch Validatoren für v.a. (syntaktische Fehler) vorhanden ()
		% http://www.rdfabout.com/demo/validator/
		% http://swse.deri.org/RDFAlerts/
	% Semantic Games : Entdecken von semantischen und logischen Fehlern  (die strukturell nicht gefunden werden können)
	% Inhaltliche Fehler (Einige Applikationen stellen Feedback-Mechanismen zur Verfügung), der Fehler wird korrigiert

	

